Human-Centric Resource Allocation in the Metaverse over Wireless Communications

The Metaverse will provide numerous immersive applications for human users, by consolidating technologies like extended reality (XR), video streaming, and cellular networks. Optimizing wireless communications to enable the human-centric Metaverse is important to satisfy the demands of mobile users. In this paper, we formulate the optimization of the system utility-cost ratio (UCR) for the Metaverse over wireless networks. Our human-centric utility measure for virtual reality (VR) applications of the Metaverse represents users' perceptual assessment of the VR video quality as a function of the data rate and the video resolution, and is learnt from real datasets. The variables jointly optimized in our problem include the allocation of both communication and computation resources as well as VR video resolutions. The system cost in our problem comprises the energy consumption and delay, and is non-convex with respect to the optimization variables due to fractions in the mathematical expressions. To solve the non-convex optimization, we develop a novel fractional programming technique, which contributes to optimization theory and has broad applicability beyond our paper. Our proposed algorithm for the system UCR optimization is computationally efficient and finds a stationary point to the constrained optimization. Through extensive simulations, our algorithm is demonstrated to outperform other approaches.

==> notused.tex <==

\begin{table}[]
\footnotesize
\caption{%\small
Notations and their meanings for solving the KKT conditions (\ref{Stationaritybn})--(\ref{Dualfeasibility}) of Problem $\mathbb{P}_{5}(\boldsymbol{z},y,\boldsymbol{s})$. The relationships between the notations are given in~(\ref{relation-bigstar-blacksquare}),~(\ref{relation-blacksquare-blacktriangle}) and~(\ref{relation-blacktriangledown-blacksquare}).
% $\blackasymbol^{\#}(\cdot)$, $\breve{\blackasymbol}(\cdot)$ and ? are given in ??, where $\blackasymbol$ can denote $\boldsymbol{b}$, $\boldsymbol{p}$, etc.
 Note that a boldfaced vector  $\boldsymbol{v}$ means $[v_n |_{n\in\mathcal{N}}]$; e.g., $\boldsymbol{b}^{\#}(\cdot) = [b_n^{\#}(\cdot) |_{n\in\mathcal{N}}]$, etc.}\label{talbenotation}
\hspace{-20pt}\setlength{\tabcolsep}{.2em}\begin{tabular}{|l|l|}
\hline
\textbf{Notation}                                                                                                                                                            & \textbf{Meaning}                                       \\ \hline
\begin{tabular}[c]{@{}l@{}} \tiny $[\boldsymbol{b}^{\#}(\bigstar),\boldsymbol{p}^{\#}(\bigstar),(\boldsymbol{f}^{\textnormal{MS}})^{\#}(\bigstar),(\boldsymbol{f}^{\textnormal{VU}})^{\#}(\bigstar),T^{\#}(\bigstar), \alpha^{\#}(\bigstar),\beta^{\#}(\bigstar),\gamma^{\#}(\bigstar),\boldsymbol{\delta}^{\#}(\bigstar)  ,\boldsymbol{\zeta}^{\#}(\bigstar)]$,\\ where ``{\tiny$ (\bigstar)$}'' means ``$(\boldsymbol{z},y,\boldsymbol{s})$''.   \end{tabular} & \begin{tabular}[c]{@{}l@{}}Given ``\textnormal{\footnotesize$\bigstar$}'', a globally optimal solution to  Problem $\mathbb{P}_{5}(\textnormal{\footnotesize$\bigstar$})$; \\i.e., a solution of  $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \alpha,\beta,\gamma,\boldsymbol{\delta}  ,\boldsymbol{\zeta}]$  to \\the KKT conditions of  Problem $\mathbb{P}_{5}(\textnormal{\footnotesize$\bigstar$})$: (\ref{Stationaritybn})--(\ref{Dualfeasibility}).\end{tabular} \\ \hline 
% \begin{tabular}[c]{@{}l@{}} ~\\[-10pt]$\grave{\zeta}_n(T\mid \textnormal{\small$\bigstar$})$ \end{tabular} & a\\ \hline
% \begin{tabular}[c]{@{}l@{}}$[\grave{\boldsymbol{b}}(\cdot),\breve{\boldsymbol{p}}(\cdot),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\cdot),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\cdot),\breve{\alpha}(\cdot),\breve{\beta}(\cdot),\breve{\gamma}(\cdot),\breve{\boldsymbol{\delta}}(\cdot)]$, \\  where ``$(\cdot)$'' means ``$(T\mid \textnormal{\small$\bigstar$})$'' \end{tabular} & \begin{tabular}[c]{@{}l@{}}A solution of $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \alpha,\gamma,\boldsymbol{\delta}  ,\boldsymbol{\zeta}]$ to \\ (\ref{Stationaritybn})--(\ref{Complementaryalpha}) and (\ref{Complementarygamma})--(\ref{Complementarytime}), \textnormal{(\ref{constraintbn})}, \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})},  \textnormal{(\ref{constraintTtau})},
% (\ref{Dualfeasibility}a), (\ref{Dualfeasibility}c), (\ref{Dualfeasibility}d), (\ref{Dualfeasibility}e)\\(i.e., the KKT conditions  (\ref{Stationaritybn})--(\ref{Dualfeasibility}) except for those related to $\beta$:\\ (\ref{Complementarybeta}), (\ref{constraintpn}), (\ref{Dualfeasibility}b)).   \end{tabular}  \\ \hline
\begin{tabular}[c]{@{}l@{}}$[\acute{\boldsymbol{b}}(\blacktriangle),\acute{\boldsymbol{p}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangle),\acute{\alpha}(\blacktriangle),\acute{\beta}(\blacktriangle),\acute{\gamma}(\blacktriangle),\acute{\boldsymbol{\delta}}(\blacktriangle)]$, \\  where ``$(\blacktriangle)$'' means ``$(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$'' \end{tabular} & \begin{tabular}[c]{@{}l@{}} Given ``$\blacktriangle$'', a globally optimal solution to   of Problem $\mathbb{P}_{66}(\blacktriangle)$; \\i.e., a solution of  $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},\alpha,\beta,\gamma,\boldsymbol{\delta} ]$ to \\ the KKT conditions of Problem $\mathbb{P}_{66}(\blacktriangle)$: \\ (\ref{Stationaritybn})--(\ref{partialLpartialfVU}), (\ref{Complementaryalpha})--(\ref{Complementarydelta}), \textnormal{(\ref{constraintbn})}, \textnormal{(\ref{constraintpn})}, \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})}, 
(\ref{Dualfeasibility}a)--(\ref{Dualfeasibility}d);\\i.e., the KKT conditions  (\ref{Stationaritybn})--(\ref{Dualfeasibility}) of $\mathbb{P}_{5}(\textnormal{\footnotesize$\bigstar$})$ except for those related \\to $T$ and $\boldsymbol{\zeta}$: (\ref{partialLpartialT}), (\ref{Complementarytime}), (\ref{constraintTtau}), (\ref{Dualfeasibility}e.   \end{tabular}  \\ \hline
\begin{tabular}[c]{@{}l@{}}$[\breve{\boldsymbol{b}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{p}}(\textnormal{\small$\blacksquare$}),
\iffalse\breve{\boldsymbol{f}}^{\textnormal{MS}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\textnormal{\small$\blacksquare$}),\fi\breve{\alpha}(\textnormal{\small$\blacksquare$})
\iffalse,\breve{\gamma}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{\delta}}(\textnormal{\small$\blacksquare$})\fi]$, \\  where ``$(\textnormal{\small$\blacksquare$})$'' means ``$(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$'' \end{tabular} & \begin{tabular}[c]{@{}l@{}}Given ``$\textnormal{\small$\blacksquare$}$'', a solution of $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},\alpha,\gamma,\boldsymbol{\delta}]$ to \\ (\ref{Stationaritybn})--(\ref{partialLpartialfVU}), (\ref{Complementaryalpha}), (\ref{Complementarygamma}), (\ref{Complementarydelta}), \textnormal{(\ref{constraintbn})}, \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})},   
(\ref{Dualfeasibility}a), (\ref{Dualfeasibility}c), (\ref{Dualfeasibility}d); \\i.e., the KKT conditions  (\ref{Stationaritybn})--(\ref{Dualfeasibility}) of $\mathbb{P}_{5}(\textnormal{\footnotesize$\bigstar$})$ except for those related \\to $\beta$, $T$ and $\boldsymbol{\zeta}$: (\ref{partialLpartialT}), (\ref{Complementarybeta}), (\ref{Complementarytime}), (\ref{constraintpn}), (\ref{constraintTtau}), (\ref{Dualfeasibility}b, (\ref{Dualfeasibility}e).   \end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}$[\widetilde{\boldsymbol{b}}(\blacktriangledown),\widetilde{\boldsymbol{p}}(\blacktriangledown),\iffalse\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangledown),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangledown), \widetilde{\gamma}(\blacktriangledown),\widetilde{\boldsymbol{\delta}}(\blacktriangledown) \fi]$, \\  where ``$(\blacktriangledown)$'' means ``$(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$''\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}A solution of $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},\gamma,\boldsymbol{\delta}]$ to \\ (\ref{Stationaritybn})--(\ref{partialLpartialfVU}), (\ref{Complementarygamma}), (\ref{Complementarydelta}), \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})},   (\ref{Dualfeasibility}c), (\ref{Dualfeasibility}d) (i.e., the KKT\\   conditions  (\ref{Stationaritybn})--(\ref{Dualfeasibility}) of $\mathbb{P}_{5}(\textnormal{\footnotesize$\bigstar$})$ except for those related to $\alpha$, $\beta$, $T$ and $\boldsymbol{\zeta}$:\\  (\ref{partialLpartialT}), (\ref{Complementaryalpha}), (\ref{Complementarybeta}), (\ref{Complementarytime}), (\ref{constraintbn}), (\ref{constraintpn}), (\ref{constraintTtau}), (\ref{Dualfeasibility}a), (\ref{Dualfeasibility}b), (\ref{Dualfeasibility}e.   \end{tabular}\\ \hline
\end{tabular}
\end{table}


======

We need to use the above to solve for $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \alpha,\beta,\gamma,\boldsymbol{\delta},\boldsymbol{\zeta}]$. Each boldfaced symbol above is an $N$-dimensional vector, so we actually need to solve for $(6N+4)$ variables. We also have $(6N+4)$ equalities, where each of (\ref{Stationaritybn})--(\ref{partialLpartialfVU}),   (\ref{Complementarydelta}) and 
 (\ref{Complementarytime}) has $N$ equalities, and each of  (\ref{partialLpartialT}), (\ref{Complementarybeta}), (\ref{Complementarygamma}) and  (\ref{Complementaryalpha}) (i.e.,  (\ref{Complementaryalpha2})) has one equality. In view of the equalities, since it is challenging to simultaneously solve for all the variables, we instead propose the following steps to compute the variables gradually (how we come up with them will be discussed soon):\vspace{10pt}
 \begin{itemize}[leftmargin=50pt]
\begin{minipage}{\linewidth} \label{substeps}
\item[\textbf{Step 2.1:}] Suppose $\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}, \boldsymbol{z},y, \boldsymbol{s}$ are given. Based on (\ref{Stationaritybn})--(\ref{partialLpartialfVU}) and (\ref{Complementarygamma}), (\ref{Complementarydelta}), \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})},   (\ref{Dualfeasibility}c), (\ref{Dualfeasibility}d), decide $\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},\gamma,\boldsymbol{\delta}$ as functions of $[\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}, \boldsymbol{z},y, \boldsymbol{s}]$.
\item[\textbf{Step 2.2:}] On top of Step 2.1, decide $\alpha$ ensuring (\ref{Complementaryalpha}), (\ref{constraintbn}) and (\ref{Dualfeasibility}a) as a function of $[\beta,\iffalse T,\fi\boldsymbol{\zeta}, \boldsymbol{z},y, \boldsymbol{s}]$.
\item[\textbf{Step 2.3:}] On top of Step 2.2, decide $\beta$ ensuring (\ref{Complementarybeta}), (\ref{constraintpn}) and (\ref{Dualfeasibility}b) as a function of $[\iffalse T,\fi\boldsymbol{\zeta}, \boldsymbol{z},y, \boldsymbol{s}]$.
\item[\textbf{Step 2.4:}] On top of Step 2.3, decide $\iffalse T,\fi\boldsymbol{\zeta}$ ensuring (\ref{partialLpartialT}), (\ref{Complementarytime}), (\ref{constraintTtau}) and (\ref{Dualfeasibility}e) as functions of $[\boldsymbol{z},y,\boldsymbol{s}]$.
\item[\textbf{Step 2.5:}] Based on the above, we can express $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \alpha,\beta,\gamma,\boldsymbol{\delta},\boldsymbol{\zeta}]$ satisfying (\ref{Stationaritybn})--(\ref{Dualfeasibility}) as functions of  $[\boldsymbol{z},y,\boldsymbol{s}]$, thus solving Problem $\mathbb{P}_{5}(\boldsymbol{z},y,\boldsymbol{s})$ globally.\vspace{10pt}   
  \end{minipage}
\end{itemize}

======
In principle, the bisection method does not need the monotonicity of the function involved. Yet, for~(\ref{betahat})?, we still provide Lemma~\ref{lemsolvebreve}? below, to better understand the obtained solution, as explained below.


% solving~(\ref{betahat}) based on the bisection method does not need the following Lemma~\ref{lemsolvebreve}. For completeness, we present it.

Theoretically, we can only show \mbox{non-increasingness} of $\sum_{n \in \mathcal{N}} \breve{p}_n(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$})$ as given in Lemma~\ref{lemsolvebreve} below since there may be degenerate cases (e.g., when all users have the same parameters). Yet, as shown in our simulation, for \mbox{non-degenerate} cases, $\sum_{n \in \mathcal{N}} \breve{p}_n(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$})$ is strictly decreasing as $\beta$ increases, which means the uniqueness of $\acute{\beta}(\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$})$ in practice, as the solution of $\beta$ to~(\ref{solvebeta1})--(\ref{solvebeta3}) given $[\boldsymbol{\zeta}, \textnormal{\small$\bigstar$}]$.

 
\begin{lemma}[Proved in Appendix~\ref{seclemsolvebreve}] \label{lemsolvebreve} 
% Given $[\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s}]$, let  $[\breve{\boldsymbol{b}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}), \breve{\alpha}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\gamma}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{\delta}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})  ,\breve{\boldsymbol{\zeta}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})]$ be a solution of $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \alpha,\gamma,\boldsymbol{\delta}  ,\boldsymbol{\zeta}]$ to (\ref{Stationaritybn})--(\ref{Complementaryalpha}) and (\ref{Complementarygamma})--(\ref{Dualfeasibility}) (\ref{Dualfeasibility}a) (\ref{Dualfeasibility}c) (\ref{Dualfeasibility}d) (\ref{Dualfeasibility}e) (i.e., the KKT conditions (\ref{Stationaritybn})--(\ref{Dualfeasibility}) except for (\ref{Complementarybeta}) and (\ref{Dualfeasibility}b)). 
Given $[\iffalse T,\fi\boldsymbol{\zeta},\textnormal{\small$\bigstar$}]$, we have that $\sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$}),\beta,\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$}) $ is \mbox{non-increasing} as $\beta$ increases.  
\end{lemma}

====


\subsection[]{The bisection method to solve the KKT conditions \ref{kktproblem5} of Problem $\mathbb{P}_{5}(\boldsymbol{z},y,\boldsymbol{s})$}

Based on ??, we use the bisection method several times to find a solution to the KKT conditions ?? of Problem $\mathbb{P}_{5}(\boldsymbol{z},y,\boldsymbol{s})$. The details are shown in Algorithms~\ref{algo:P5}, ??, and ??.
In principle, the bisection method does not require the monotonicity of the function to be evaluated. Yet, we still provide Propositions ??-?? below to obtain the following insight. Although  theoretically we show only ``\mbox{non-increasing}'' instead of ``\mbox{decreasing}'' in Propositions ?? and ??, in practice, as long as the considered scenario is not degenerate, we actually have ``\mbox{decreasing}'' for Propositions ??-??. Since the bisection method for monotone functions has only one root, we get the insight that in \mbox{non-degenerate} scenarios in practice, there is exactly one globally optimal solution $[\boldsymbol{b}^{\#}(\boldsymbol{z},y,\boldsymbol{s}),\boldsymbol{p}^{\#}(\boldsymbol{z},y,\boldsymbol{s}),(\boldsymbol{f}^{\textnormal{MS}})^{\#}(\boldsymbol{z},y,\boldsymbol{s}),(\boldsymbol{f}^{\textnormal{VU}})^{\#}(\boldsymbol{z},y,\boldsymbol{s}),T^{\#}(\boldsymbol{z},y,\boldsymbol{s})]$ to Problem $\mathbb{P}_{5}(\boldsymbol{z},y,\boldsymbol{s})$, which our Algorithm~\ref{algo:P5} can find at convergence.


% Yet, our Propositions ??-?? show that in practice, as long as the 

\begin{lemma}[Proved in Appendix~\ref{seclemsolvepngivenalphaandbeta}] \label{lemsolvepngivenalphaandbeta}
Given $[\alpha,\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s}]$, the left hand side of~(\ref{solvepngivenalphaandbeta}) is \mbox{decreasing} as $\zeta_n$ increases.  ? $h_n(\boldsymbol{\zeta}\mid T)$
\end{lemma}



We define $\grave{\zeta}_n(T\mid \boldsymbol{z},y, \boldsymbol{s})$ as the solution of $\zeta_n$ such that
\begin{align}
t_n(\acute{b}_n(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{p}_n(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s}),s_n,\acute{f}_n^{\textnormal{MS}}(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{f}_n^{\textnormal{VU}}(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s})) = T.    
\end{align}
Since ?? is \mbox{non-increasing} as $\zeta_n$ increases, we know that $\grave{\zeta}_n(T\mid \boldsymbol{z},y, \boldsymbol{s})$ is \mbox{non-increasing} as $T$ increases.

We define $T^{\#}(\boldsymbol{z},y,\boldsymbol{s})$ as the solution of $T$ such that
\begin{align}
\sum_{n \in \mathcal{N}} \max\{\grave{\zeta}_n(T\mid \boldsymbol{z},y, \boldsymbol{s}), 0\} = y c_{\hspace{0.8pt}\textnormal{t}}.    
\end{align}



% \begin{proposition} 
% \begin{itemize}
% \item 
% \item Given $\beta$, $\widetilde{p}_n(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$ is a strictly increasing function in $\alpha$.
% \item Given $\alpha$, $\widetilde{p}_n(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$ is a strictly decreasing function in $\beta$.
% \end{itemize}

% \end{proposition}

We define $\breve{\alpha}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z}, y, \boldsymbol{s})$ as a solution of $\alpha$ to ensuring

Then $\beta^{\#}(y, \boldsymbol{z})$ is defined as a solution of $\beta$ to ensuring
\begin{align} 
\beta \cdot \bigg( \sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s}),\beta \mid \boldsymbol{z},y, \boldsymbol{s}) - p_{\textnormal{max}}\bigg) = 0. \label{betahash2}
\end{align} 

\begin{align} 
 \sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s}),\beta \mid \boldsymbol{z},y, \boldsymbol{s}) - p_{\textnormal{max}} = 0. \label{betahash}
\end{align} 

With $\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s})$ defined above, for convenience, we define
\begin{subnumcases}{} 
\breve{b}_n(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}): = \widetilde{b}_n(\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s}),\beta \mid y, z_n) \textnormal{ defined in ??},   \\  \breve{p}_n(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}): = \widetilde{p}_n(\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s}),\beta \mid y, z_n) \textnormal{ defined in ??}, . \\  \breve{f}^{\textnormal{MS}}_n(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}): = \\ \breve{f}^{\textnormal{VU}}_n(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}): =
\end{subnumcases} 
 

\begin{proposition} 
$\alpha^*$ and $\beta^*$ satisfying ??, ?? and ?? are solutions of $\alpha$ and $\beta$ to
\begin{subnumcases}{} 
 \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha,\beta \mid \boldsymbol{z},y)  = b_{\textnormal{max}} ,   \\  \beta \cdot \bigg( \sum_{n \in \mathcal{N}} \widetilde{p}_n(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) - p_{\textnormal{max}}\bigg) = 0.
\end{subnumcases} 

\end{proposition}

 

Case 1: If $\beta = 0$,
then 
\begin{align} 
 \sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(0\mid \boldsymbol{z},y, \boldsymbol{s}),0 \mid \boldsymbol{z},y, \boldsymbol{s}) \leq p_{\textnormal{max}} \label{conditionbeta0}
\end{align} 
% We need to show if \begin{align} 
%  \sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s}),\beta \mid y, z_n) = p_{\textnormal{max}}
% \end{align} 
% then
% $\beta \leq 0$

Case 2: If $\beta > 0$,
\begin{align} 
 \sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s}),\beta \mid \boldsymbol{z},y, \boldsymbol{s}) = p_{\textnormal{max}}
\end{align} 
We need to show
\begin{align} 
 \sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(0\mid y, \boldsymbol{z}),0 \mid \boldsymbol{z},y, \boldsymbol{s}) > p_{\textnormal{max}}
\end{align}

\begin{subnumcases}{} 
\textnormal{If }\sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(0\mid y, \boldsymbol{z}),0 \mid \boldsymbol{z},y, \boldsymbol{s}) \leq p_{\textnormal{max}}, \textnormal{then } \begin{cases}\widehat{\beta}(y, \boldsymbol{z}) = 0, \\ \widehat{\alpha}(y, \boldsymbol{z}) = \breve{\alpha}(0\mid y, \boldsymbol{z}), \\  \widehat{b}_n(y, \boldsymbol{z})= \widetilde{b}_n(\breve{\alpha}(0\mid y, \boldsymbol{z}),0 \mid y, z_n), \\  \widehat{p}_n(y, \boldsymbol{z})= \widetilde{p}_n(\breve{\alpha}(0\mid y, \boldsymbol{z}),0 \mid \boldsymbol{z},y, \boldsymbol{s}),  \end{cases}   \\ \textnormal{If }\sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(0\mid y, \boldsymbol{z}),0 \mid \boldsymbol{z},y, \boldsymbol{s}) > p_{\textnormal{max}}, \textnormal{then } \begin{cases}\widehat{b}_n(y, \boldsymbol{z}) \textnormal{ is a solution of $\beta$ to} \\  \sum_{n \in \mathcal{N}} \widetilde{p}_n(\breve{\alpha}(\beta\mid \boldsymbol{z}, y, \boldsymbol{s}),\beta \mid y, z_n) = p_{\textnormal{max}}, \\  \widehat{\alpha}(y, \boldsymbol{z}) = a(\hspace{1pt}\widehat{b}_n(y, \boldsymbol{z})\mid y, \boldsymbol{z}),  \\ \widehat{b}_n(y, \boldsymbol{z})= \widetilde{b}_n(a(\hspace{1pt}\widehat{b}_n(y, \boldsymbol{z})\mid y, \boldsymbol{z}),0 \mid y, z_n), \\  \widehat{p}_n(y, \boldsymbol{z})= \widetilde{p}_n(a(\hspace{1pt}\widehat{b}_n(y, \boldsymbol{z})\mid y, \boldsymbol{z}),0 \mid y, z_n),  \end{cases}  
\end{subnumcases} 


we let $\overline{\alpha}(y, \boldsymbol{z})$ (abbreviated as $\overline{\alpha}$ sometimes for simplicity) be 
a solution of $\alpha> 0$ to $ \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha,0 \mid y, z_n)  = b_{\textnormal{max}}$; i.e., 
\begin{subnumcases}{} 
\sum_{n \in \mathcal{N}} \widetilde{b}_n(\overline{\alpha},0 \mid y, z_n)  = b_{\textnormal{max}} ,   \\  \sum_{n \in \mathcal{N}} \widetilde{p}_n(\overline{\alpha},0 \mid y, z_n) \leq p_{\textnormal{max}}.
\end{subnumcases}
Then satisfies $\sum_{n \in \mathcal{N}} \widetilde{p}_n(\alpha,0 \mid y, z_n) \leq p_{\textnormal{max}}$.




Case 2: If $\beta > 0$,
then we let $\widehat{\alpha}(y, \boldsymbol{z}) > 0$ and $\widehat{\beta}(y, \boldsymbol{z}) > 0$ (abbreviated as $\widehat{\alpha}$ and $\widehat{\beta}$ sometimes for simplicity) be 
solutions of $\alpha$ and $\beta$ to
\begin{subnumcases}{} 
 \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha,\beta \mid \boldsymbol{z},y)  = b_{\textnormal{max}} ,   \\  \sum_{n \in \mathcal{N}} \widetilde{p}_n(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) = p_{\textnormal{max}}.
\end{subnumcases}

 a solution of $\alpha$ to $ \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha,0 \mid y, z_n)  = b_{\textnormal{max}}$ satisfies $\sum_{n \in \mathcal{N}} \widetilde{p}_n(\alpha,0 \mid y, z_n) > p_{\textnormal{max}}$

Let $\overline{\alpha}$ be 
a solution of $\alpha$ to $ \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha,0 \mid y, z_n)  = b_{\textnormal{max}}$

====


\begin{align}
\textnormal{Problem $\mathbb{P}_{66}(\iffalse T,\fi\boldsymbol{\zeta}\mid\boldsymbol{z},y,\boldsymbol{s})$}:\min_{\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}}} \quad & -H_{\mathbb{P}_{5}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},0\mid \boldsymbol{z},y,\boldsymbol{s})  +\sum_{n \in \mathcal{N}} \Big(\zeta_n  t_n(b_n,p_n,s_n,f_n^{\textnormal{MS}},f_n^{\textnormal{VU}}) \Big) \label{eqP5} \\
\textrm{s.t.} \quad &  \textnormal{(\ref{constraintbn})}, \textnormal{(\ref{constraintpn})}, \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})} 
\end{align} 


\appendix

\subsection{Proof of Lemma~\ref{lemsolvepngivenalphaandbeta}} \label{seclemsolvepngivenalphaandbeta}

 
  
First, we note $\alpha > 0$ from Step~1 on Page~\pageref{step1}. Then from~(\ref{definepsin}), we know (i) $\psi_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s})$ is positive and decreasing in $p_n$. In addition, (ii) the function $\log_2(1+x) - \frac{x}{(1+x) \ln 2}$ is increasing and positive   for $x>0$ since the derivative $\frac{x}{(1+x)^2 \ln 2}$ is positive for $x>0$, and $\log_2(1+x) - \frac{x}{(1+x) \ln 2}$ at $x=0$ equals $0$. From the above Results ``(i)'' and ``(ii)'', we obtain (iii) $\left[
    \log_2\big(1+\psi_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s})\big)
     -\frac{\psi_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s})}{(1+\psi_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s}))\ln2}\right]$ is positive and decreasing  in $p_n$.

We also have (iv) the function $\frac{\log_2(1+x)}{x}$ is decreasing for $x>0$ since the derivative $\frac{1}{x^2}[\frac{x}{(1+x) \ln 2} - \log_2(1+x)]  $ is negative due to Result ``(ii)'' above. From the above Results ``(i)'' and ``(iv)'', we obtain (v) $\overline{r}_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s})$ defined in~(\ref{eqdefinernoverline}) is increasing in $p_n$. Since the utility function $U_n(r_n, s_n)$ is concave and \mbox{non-decreasing} in $r_n$, $\frac{\partial U_n(r_n, s_n)}{\partial r_n}$ is \mbox{non-negative} and \mbox{non-increasing} in $r_n$. Then (vi) $ \frac{\partial U_n(r_n, s_n)}{\partial r_n}   + \frac{y}{2z_n{r_n}^3}  + \frac{\zeta   s_n}{{r_n}^2} $ is positive and \mbox{non-increasing} in $r_n$. From the above Results ``(v)'' and ``(vi)'', we obtain (vii) $\big(\frac{\partial U_n(r_n, s_n)}{\partial r_n}\big)|_{r_n=\overline{r}_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s})}    + \frac{y}{2z_n \cdot [\overline{r}_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s})]^3}   + \frac{\zeta_n s_n}{ [\overline{r}_n(p_n,\alpha,\beta \mid \boldsymbol{z},y, \boldsymbol{s})]^2}$ is positive and \mbox{non-increasing} in $p_n$.

From the above Results ``(iii)'' and ``(vii)'', the left hand side of~(\ref{solvepngivenalphaandbeta}) is \mbox{decreasing} as $p_n$ increases.  \qed


\subsection{Proof of Lemma~\ref{lemsolvebreve}} \label{seclemsolvebreve}

From Lemma~\ref{lemsolvebreve}'s condition, setting $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \alpha,\gamma,\boldsymbol{\delta}  ,\boldsymbol{\zeta}]$ as
$[\breve{\boldsymbol{b}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}), \breve{\alpha}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\gamma}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{\delta}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})  ,\breve{\boldsymbol{\zeta}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})]$ satisfies (\ref{Stationaritybn})--(\ref{Complementaryalpha}) and (\ref{Complementarygamma})--(\ref{Dualfeasibility}). It is straightforward to see that (\ref{Stationaritybn})--(\ref{Complementaryalpha}) and (\ref{Complementarygamma})--(\ref{Dualfeasibility}) are exactly the KKT conditions to the following Problem $\mathbb{P}_{6}(\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$: 
\begin{align}
\textnormal{Problem $\mathbb{P}_{6}(\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$}: \min_{\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T} \quad & -H_{\mathbb{P}_{5}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \boldsymbol{z},y,\boldsymbol{s})  + \beta \cdot \big( \sum_{n \in \mathcal{N}} p_n - p_{\textnormal{max}}\big)   \\
\textrm{s.t.} \quad &  \textnormal{(\ref{constraintbn})}, \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})},  \textnormal{(\ref{constraintTtau})} , \label{eqP6}
\end{align} 
where $H_{\mathbb{P}_{5}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \boldsymbol{z},y,\boldsymbol{s})$ denotes the objective function of $\mathbb{P}_{5}(\boldsymbol{z},y,\boldsymbol{s})$ in~(\ref{eqP5}).
Hence,
\begin{align}
\begin{array}{l}
\text{$[\breve{\boldsymbol{b}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})]$} \\  \text{is a globally optimal solution to $\mathbb{P}_{6}(\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$.}    
\end{array} \label{P6result}   
\end{align}

 
 
To prove Lemma~\ref{lemsolvebreve}, we consider the case where $\beta$ equals $\beta_1$, and the case where $\beta$ equals $\beta_2$, respectively, for arbitrarily chosen $\beta_1$ and $\beta_2$. Due to Result~(\ref{P6result}) above, we obtain
\begin{align}
&H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_1, \boldsymbol{z},y, \boldsymbol{s}) \nonumber \\ & \leq H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_1, \boldsymbol{z},y, \boldsymbol{s})  , \label{eqbeta1beta21}
\end{align}
and
\begin{align}
&H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_2, \boldsymbol{z},y, \boldsymbol{s}) \nonumber \\ & \leq H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_2, \boldsymbol{z},y, \boldsymbol{s}) .\label{eqbeta1beta22}  
\end{align}
From~(\ref{eqbeta1beta21}) and~(\ref{eqbeta1beta22}), it follows that
\begin{align}
& \left[ \begin{array}{l}
H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_1, \boldsymbol{z},y, \boldsymbol{s})   \\   - H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_2, \boldsymbol{z},y, \boldsymbol{s})  
\end{array} \right] \nonumber \\ & + \left[ \begin{array}{l}
H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_2, \boldsymbol{z},y, \boldsymbol{s})   \\   - H_{\mathbb{P}_{6}}(\breve{\boldsymbol{b}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{p}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}),\breve{T}(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \beta_1, \boldsymbol{z},y, \boldsymbol{s})  
\end{array} \right] \leq 0.  \label{eqbeta1beta2} 
\end{align}
Since $H_{\mathbb{P}_{6}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$ equals $-H_{\mathbb{P}_{5}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \boldsymbol{z},y,\boldsymbol{s})  + \beta \cdot \big( \sum_{n \in \mathcal{N}} p_n - p_{\textnormal{max}}\big) $ from~(\ref{eqP6}), the term inside the first ``$[\cdot]$'' of~(\ref{eqbeta1beta2}) equals $(\beta_1 - \beta_2) \cdot \big( \sum_{n \in \mathcal{N}} \breve{p}_n(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}) - p_{\textnormal{max}}\big)$, and the term inside the second ``$[\cdot]$'' of~(\ref{eqbeta1beta2}) equals $(\beta_2 - \beta_1) \cdot \big( \sum_{n \in \mathcal{N}} \breve{p}_n(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}) - p_{\textnormal{max}}\big)$. Then we obtain
\begin{align}
(\beta_1 - \beta_2) \cdot \big( \sum_{n \in \mathcal{N}} \breve{p}_n(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}) - p_{\textnormal{max}}\big) + (\beta_2 - \beta_1) \cdot \big( \sum_{n \in \mathcal{N}} \breve{p}_n(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}) - p_{\textnormal{max}}\big) \leq 0;   
\end{align}
i.e., $(\beta_1 - \beta_2) \cdot \big( \sum_{n \in \mathcal{N}} \breve{p}_n(\beta_1\mid \boldsymbol{z},y, \boldsymbol{s}) - \sum_{n \in \mathcal{N}} \breve{p}_n(\beta_2\mid \boldsymbol{z},y, \boldsymbol{s}) \big) \leq 0$. Hence, given $[\boldsymbol{z},y, \boldsymbol{s}]$, $\sum_{n \in \mathcal{N}} \breve{p}_n(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$ is \mbox{non-increasing} as $\beta$ increases. \qed

 \subsection{Proof of Proposition~\ref{lemsolvewidetilde}} \label{seclemsolvewidetilde}

From Proposition~\ref{lemsolvewidetilde}'s condition, setting $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \gamma,\boldsymbol{\delta}  ,\boldsymbol{\zeta}]$ as
$[\widetilde{\boldsymbol{b}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}), \widetilde{\gamma}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{\delta}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})  ,\widetilde{\boldsymbol{\zeta}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})]$ satisfies (\ref{Stationaritybn})--(\ref{partialLpartialT}) and (\ref{Complementarygamma})--(\ref{Dualfeasibility}). It is straightforward to see that (\ref{Stationaritybn})--(\ref{partialLpartialT}) and (\ref{Complementarygamma})--(\ref{Dualfeasibility}) are exactly the KKT conditions to the following Problem $\mathbb{P}_{7}(\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$: 
\begin{align}
\textnormal{Problem $\mathbb{P}_{7}(\alpha,\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$}: \min_{\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T} \quad & -H_{\mathbb{P}_{6}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \beta,\boldsymbol{z},y,\boldsymbol{s}) + \alpha \cdot \bigg( \sum_{n \in \mathcal{N}} b_n - b_{\textnormal{max}}\bigg)     \\
\textrm{s.t.} \quad &   \textnormal{(\ref{constraintfMS})}, \textnormal{(\ref{constraintfn})},  \textnormal{(\ref{constraintTtau})} , \label{alphaeqP6}
\end{align} 
where $H_{\mathbb{P}_{6}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \beta,\boldsymbol{z},y,\boldsymbol{s})$ denotes the objective function of $\mathbb{P}_{6}(\beta,\boldsymbol{z},y,\boldsymbol{s})$ in~(\ref{eqP6}).
Hence, 
\begin{align}
\begin{array}{l}
\text{$[\widetilde{\boldsymbol{b}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})]$} \\  \text{is a globally optimal solution to $\mathbb{P}_{7}(\alpha,\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$.}    
\end{array} \label{P7result}   
\end{align} 
 
To prove Proposition~\ref{lemsolvewidetilde}, we consider the case where $\alpha$ equals $\alpha_1$, and the case where $\alpha$ equals $\alpha_2$, respectively, for arbitrarily chosen $\alpha_1$ and $\alpha_2$. Due to Result~(\ref{P7result}) above, we obtain
\begin{align} 
&\resizebox{1\hsize}{!}{$H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$} \nonumber \\ & \resizebox{1\hsize}{!}{$\leq H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$}   , \label{alphaeqalpha1alpha21}
\end{align}
and
\begin{align}
&\resizebox{1\hsize}{!}{$H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_2, \beta,\boldsymbol{z},y, \boldsymbol{s})$}  \nonumber \\ & \resizebox{1\hsize}{!}{$\leq H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_2, \beta,\boldsymbol{z},y, \boldsymbol{s}) .$} \label{alphaeqalpha1alpha22}  
\end{align}
From~(\ref{alphaeqalpha1alpha21}) and~(\ref{alphaeqalpha1alpha22}), it follows that
\begin{align}
& \resizebox{1\hsize}{!}{$\left[ \begin{array}{l}
H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_1, \boldsymbol{z},y, \boldsymbol{s})   \\   - H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_2, \beta,\boldsymbol{z},y, \boldsymbol{s})  
\end{array} \right]$} \nonumber \\ & \resizebox{1\hsize}{!}{$+ \left[ \begin{array}{l}
H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_2, \beta,\boldsymbol{z},y, \boldsymbol{s})   \\   - H_{\mathbb{P}_{7}}(\widetilde{\boldsymbol{b}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{p}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \mid \alpha_1, \boldsymbol{z},y, \boldsymbol{s})  
\end{array} \right] \leq 0.$}  \label{alphaeqalpha1alpha2} 
\end{align}
Since $H_{\mathbb{P}_{7}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \alpha,\beta,\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s})$ equals $-H_{\mathbb{P}_{6}}(\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T \mid \beta,\boldsymbol{z},y,\boldsymbol{s}) + \alpha \cdot \big( \sum_{n \in \mathcal{N}} p_n - b_{\textnormal{max}}\big) $ from~(\ref{alphaeqP6}), the term inside the first ``$[\cdot]$'' of~(\ref{alphaeqalpha1alpha2}) equals $(\alpha_1 - \alpha_2) \cdot \big( \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) - b_{\textnormal{max}}\big)$, and the term inside the second ``$[\cdot]$'' of~(\ref{alphaeqalpha1alpha2}) equals $(\alpha_2 - \alpha_1) \cdot \big( \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) - b_{\textnormal{max}}\big)$. Then we obtain
\begin{align}
(\alpha_1 - \alpha_2) \cdot \big( \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) - b_{\textnormal{max}}\big) + (\alpha_2 - \alpha_1) \cdot \big( \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) - b_{\textnormal{max}}\big) \leq 0;   
\end{align}
i.e., $(\alpha_1 - \alpha_2) \cdot \big( \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha_1,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) - \sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha_2,\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}) \big) \leq 0$. Hence, given $[ \beta,\boldsymbol{z},y, \boldsymbol{s}]$, we have that $\sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$ is \mbox{non-increasing} as $\alpha$ increases.  \qed

 =========


 \textbf{Relationships between the notations for Steps 2.1--2.5.}

 
\begin{align}
\begin{array}{l}
 \textnormal{Given $[ \boldsymbol{z},y, \boldsymbol{s}]$,  \textbf{if} $\boldsymbol{\zeta}$ satisfies that with  $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}}, \alpha,\beta,\gamma,\boldsymbol{\delta}  ]$ being set as }  \\ \textnormal{$[\acute{\boldsymbol{b}}(\blacktriangle),\acute{\boldsymbol{p}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangle),\acute{\alpha}(\blacktriangle),\acute{\beta}(\blacktriangle),\acute{\gamma}(\blacktriangle),\acute{\boldsymbol{\delta}}(\blacktriangle)]$, there exists $T$ such that}  \\ \textnormal{(\ref{partialLpartialT}), (\ref{Complementarytime}), (\ref{constraintTtau}) and (\ref{Dualfeasibility}e) all hold, where ``$(\blacktriangle)$'' means ``$(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$'',} \\ \textnormal{\textbf{then} $[\acute{\boldsymbol{b}}(\blacktriangle),\acute{\boldsymbol{p}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangle),T,\acute{\alpha}(\blacktriangle),\acute{\beta}(\blacktriangle),\acute{\gamma}(\blacktriangle),\acute{\boldsymbol{\delta}}(\blacktriangle),\boldsymbol{\zeta}]$ will become}\\ \textnormal{$[\boldsymbol{b}^{\#}(\textnormal{\small$\bigstar$}),\boldsymbol{p}^{\#}(\textnormal{\small$\bigstar$}),(\boldsymbol{f}^{\textnormal{MS}})^{\#}(\textnormal{\small$\bigstar$}),(\boldsymbol{f}^{\textnormal{VU}})^{\#}(\textnormal{\small$\bigstar$}),T^{\#}(\textnormal{\small$\bigstar$}), \alpha^{\#}(\textnormal{\small$\bigstar$}),\beta^{\#}(\textnormal{\small$\bigstar$}),\gamma^{\#}(\textnormal{\small$\bigstar$}),\boldsymbol{\delta}^{\#}(\textnormal{\small$\bigstar$})  ,\boldsymbol{\zeta}^{\#}(\textnormal{\small$\bigstar$})]$,}\\ \textnormal{where ``{\small$ (\bigstar)$}'' means ``$(\boldsymbol{z},y,\boldsymbol{s})$''. }   
\end{array} \label{relation-bigstar-blacksquare}
\end{align}

\begin{align}
\begin{array}{l}
 \textnormal{Given $[\iffalse T,\fi\boldsymbol{\zeta}, \boldsymbol{z},y, \boldsymbol{s}]$, \textbf{if} $\beta$ satisfies that setting $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},\alpha,\gamma,\boldsymbol{\delta}]$ as }  \\ \textnormal{$[\breve{\boldsymbol{b}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{p}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\textnormal{\small$\blacksquare$}),\breve{\alpha}(\textnormal{\small$\blacksquare$}),\breve{\gamma}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{\delta}}(\textnormal{\small$\blacksquare$})]$ ensures (\ref{Complementarybeta}), (\ref{constraintpn}) and (\ref{Dualfeasibility}b),}  \\ \textnormal{where ``$(\textnormal{\small$\blacksquare$})$'' means ``$(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$'',} \\ \textnormal{\textbf{then} $[\breve{\boldsymbol{b}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{p}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\textnormal{\small$\blacksquare$}),\breve{\alpha}(\textnormal{\small$\blacksquare$}),\beta,\breve{\gamma}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{\delta}}(\textnormal{\small$\blacksquare$})]$ will become}\\ \textnormal{$[\acute{\boldsymbol{b}}(\blacktriangle),\acute{\boldsymbol{p}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangle),\acute{\alpha}(\blacktriangle),\acute{\beta}(\blacktriangle),\acute{\gamma}(\blacktriangle),\acute{\boldsymbol{\delta}}(\blacktriangle)]$,}\\ \textnormal{where ``$(\blacktriangle)$'' means ``$(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$''.}   
\end{array} \label{relation-blacksquare-blacktriangle}
\end{align}

\begin{align}
\begin{array}{l}
 \textnormal{Given $[\beta,\iffalse T,\fi\boldsymbol{\zeta}, \boldsymbol{z},y, \boldsymbol{s}]$, \textbf{if} $\alpha$ satisfies that setting $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},\gamma,\boldsymbol{\delta}]$ as }  \\ \textnormal{$[\widetilde{\boldsymbol{b}}(\blacktriangledown),\widetilde{\boldsymbol{p}}(\blacktriangledown),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangledown),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangledown),\widetilde{\gamma}(\blacktriangledown),\widetilde{\boldsymbol{\delta}}(\blacktriangledown) ]$ ensures (\ref{Complementaryalpha}), (\ref{constraintbn}) and (\ref{Dualfeasibility}a),}  \\ \textnormal{where ``$(\blacktriangledown)$'' means ``$(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$'',} \\ \textnormal{\textbf{then} $[\widetilde{\boldsymbol{b}}(\blacktriangledown),\widetilde{\boldsymbol{p}}(\blacktriangledown),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangledown),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangledown),\alpha, \widetilde{\gamma}(\blacktriangledown),\widetilde{\boldsymbol{\delta}}(\blacktriangledown) ]$ will become}\\ \textnormal{$[\breve{\boldsymbol{b}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{p}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\textnormal{\small$\blacksquare$}),\breve{\alpha}(\textnormal{\small$\blacksquare$}),\breve{\gamma}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{\delta}}(\textnormal{\small$\blacksquare$})]$,}\\ \textnormal{where ``$(\textnormal{\small$\blacksquare$})$'' means ``$(\beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$''.}   
\end{array} \label{relation-blacktriangledown-blacksquare}
\end{align}

  =========

After obtaining $\acute{\beta}(\blacktriangle)$ by solving~(\ref{solvebeta1})--(\ref{solvebeta3}), we let the $\beta$ parameter in \newline $[\breve{\boldsymbol{b}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{p}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{MS}}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{f}}^{\textnormal{VU}}(\textnormal{\small$\blacksquare$}),\breve{\alpha}(\textnormal{\small$\blacksquare$}),\breve{\gamma}(\textnormal{\small$\blacksquare$}),\breve{\boldsymbol{\delta}}(\textnormal{\small$\blacksquare$})]$ be $\acute{\beta}(\blacktriangle)$, and the corresponding results become\newline  $[\acute{\boldsymbol{b}}(\blacktriangle),\acute{\boldsymbol{p}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{MS}}(\blacktriangle),\acute{\boldsymbol{f}}^{\textnormal{VU}}(\blacktriangle),\acute{\alpha}(\blacktriangle),\acute{\gamma}(\blacktriangle),\acute{\boldsymbol{\delta}}(\blacktriangle)]$.  

 
\textbf{Section~\ref{solvetalbenotation}-4: Solving for the ``$(\textnormal{\small$\bigstar$})$'' notations (i.e., Details for Page~\pageref{substeps}'s ``Step 2.4'' and ``Step 2.5'').} Based on~(\ref{relation-bigstar-blacksquare}), we obtain the ``$(\textnormal{\small$\bigstar$})$'' (i.e., ``$(\boldsymbol{z},y,\boldsymbol{s})$'') notations by enforcing (\ref{partialLpartialT}), (\ref{Complementarytime}), (\ref{constraintTtau}) and (\ref{Dualfeasibility}e) on the ``$(\textnormal{$\blacktriangle$})$'' (i.e., ``$(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})$'') notations; i.e.,


Given ``$\textnormal{\small$\bigstar$}$'', the solution of $[T,\boldsymbol{\zeta}]$ to~(\ref{solveTzeta1})--(\ref{solveTzeta4}) is just $[T^{\#}(\textnormal{\small$\bigstar$}),\boldsymbol{\zeta}^{\#}(\textnormal{\small$\bigstar$})]$ (i.e., $[T^{\#}(\boldsymbol{z},y,\boldsymbol{s}),\boldsymbol{\zeta}^{\#}(\boldsymbol{z},y,\boldsymbol{s})]$). To solve~(\ref{solveTzeta1})--(\ref{solveTzeta4}), we present Proposition~\ref{lemsolveacute} below. 
\begin{proposition}[Proved in Appendix~\ref{seclemsolveacute}] \label{lemsolveacute} 
% Given $[\iffalse T,\fi\boldsymbol{\zeta},\boldsymbol{z},y, \boldsymbol{s}]$, let  $[\acute{\boldsymbol{b}}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{\boldsymbol{p}}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{\boldsymbol{f}}^{\textnormal{MS}}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{\boldsymbol{f}}^{\textnormal{VU}}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{\alpha}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{\beta}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{\gamma}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{\boldsymbol{\delta}}(\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})]$ be a solution of $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \alpha,\beta,\gamma,\boldsymbol{\delta}  ]$ to (\ref{Stationaritybn})--(\ref{Complementaryalpha}) and (\ref{Complementarygamma})--(\ref{Dualfeasibility}) (\ref{Dualfeasibility}a) (\ref{Dualfeasibility}c) (\ref{Dualfeasibility}d) (\ref{Dualfeasibility}e) (i.e., the KKT conditions (\ref{Stationaritybn})--(\ref{Dualfeasibility}) except for (\ref{Complementarybeta}) and (\ref{Dualfeasibility}b)).  
Given $[T,\boldsymbol{z},y, \boldsymbol{s}]$, we have that $t_n(\acute{b}_n(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{p}_n(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s}),s_n,\acute{f}_n^{\textnormal{MS}}(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s}),\acute{f}_n^{\textnormal{VU}}(T,\zeta_n\mid \boldsymbol{z},y, \boldsymbol{s}))$ is \mbox{non-increasing} as $\zeta_n$ increases.  
\end{proposition}



with


======

To better understand  the  bisection search process,
% of solving~(\ref{brevealpha}) given in Line~?? of Algorithm~??, 
we present Proposition~\ref{lemsolvewidetilde} below.

\begin{proposition}[Proved in Appendix~\ref{seclemsolvewidetilde}] \label{lemsolvewidetilde} 
% Given $[\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta},\textnormal{\small$\bigstar$}]$, let  $[\widetilde{\boldsymbol{b}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$}),\widetilde{\boldsymbol{p}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$}),\widetilde{\boldsymbol{f}}^{\textnormal{MS}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$}),\widetilde{\boldsymbol{f}}^{\textnormal{VU}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{T}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}), \widetilde{\gamma}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s}),\widetilde{\boldsymbol{\delta}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})  ,\widetilde{\boldsymbol{\zeta}}(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \boldsymbol{z},y, \boldsymbol{s})]$ be a solution of $[\boldsymbol{b},\boldsymbol{p},\boldsymbol{f}^{\textnormal{MS}},\boldsymbol{f}^{\textnormal{VU}},T, \gamma,\boldsymbol{\delta}  ,\boldsymbol{\zeta}]$ to (\ref{Stationaritybn})--(\ref{partialLpartialT}) and (\ref{Complementarygamma})--(\ref{Dualfeasibility}) (i.e., the KKT conditions (\ref{Stationaritybn})--(\ref{Dualfeasibility}) except for (\ref{Complementaryalpha}) and (\ref{Complementarybeta})).  
Given $[\beta,\iffalse T,\fi\boldsymbol{\zeta}, \textnormal{\small$\bigstar$}]$, we have that $\sum_{n \in \mathcal{N}} \widetilde{b}_n(\alpha, \beta,\iffalse T,\fi\boldsymbol{\zeta}\mid \textnormal{\small$\bigstar$})$ is \mbox{non-increasing} as $\alpha$ increases.  
\end{proposition}



